Distilling the Knowledge of Large-scale Generative Models into Retrieval Models for Efficient Open-domain Conversation

Despite the remarkable performance of large-scale generative models in open-domain conversation, they are known to be less practical for building real-time conversation systems due to high latency. On the other hand, retrieval models could return responses with much lower latency but show inferior performance to the large-scale generative models since the conversation quality is bounded by the pre-defined response set. To take advantage of both approaches, we propose a new training method called G2R (Generative-to-Retrieval distillation) that preserves the efficiency of a retrieval model while leveraging the conversational ability of a large-scale generative model by infusing the knowledge of the generative model into the retrieval model. G2R consists of two distinct techniques of distillation: the data-level G2R augments the dialogue dataset with additional responses generated by the large-scale generative model, and the model-level G2R transfers the response quality score assessed by the generative model to the score of the retrieval model by the knowledge distillation loss. Through extensive experiments including human evaluation, we demonstrate that our retrieval-based conversation system trained with G2R shows a substantially improved performance compared to the baseline retrieval model while showing significantly lower inference latency than the large-scale generative models.

==> Algorithms/algorithm_hard_negative.tex <==
\begin{algorithm}[t]
\SetAlgoLined
\SetKwInOut{Input}{input} \SetKwInOut{Output}{output}

\Input{ Retrieval Model $\mathcal{R}$, Generative Model $\mathcal{R}$, Dialogue dataset $D^\mathcal{G}$, number of loop $l$}
\Output{ Fine-tuned Retrieval model $\mathcal{R}$}
 \For{idx$\leftarrow 1$ \KwTo $l$}{
  \For{i$\leftarrow 1$ \KwTo $n$}{
    r 
  }
  \eIf{condition}{
   instructions1\;
   instructions2\;
   }{
   instructions3\;
  }
 }
 \caption{Hard-negative Correction.}
\end{algorithm}


==> Sections/999_Notepad.tex <==
%%% Section 2.3 First Draft


% Retrieval model의 문제점: Training set에 있는 말만 해야해서 Diverse한 말이 어렵다. 또한 Retrieval model을 학습할만한 데이터가 부족하거나 더 많은 데이터를 통해 이득을 볼 수 있다. 이미 학습된 Large generative model은 Ground truth에 비견할만한 답변을 만들어낼 수 있으니, 이 지식을 Retrieval model로 잘 옮겨주자!
% We denote given training dialogue as $D = \{(c_1, r_1), \cdots, (c_n, r_n)\}$ with $n$ examples, where $c_i$ is $i$-th input context and $r_i$ is a corresponding gold response.
% Models for retrieval chatbots are then trained by using $D$ as positive examples, and the pre-defined response set $R$ for inference is set to $R = \{r_1, r_2, \cdots, r_n\}$.
% Moreover, performance of the models for retrieval itself could be further developed by learning from additional positive examples as shown in \citet{zhang2020dialoguedistillation}.

% The major limitation of retrieval models is that they can only respond with the responses in the pre-defined response repository $R$, which could not be diverse enough in terms of topic, dialog act, expression, and etc [cite].

% Here, we concentrate on utilizing large-scale generative models for improving retrieval models.
% As shown in \citet{zhang2020dialoguedistillation}, the performance of retrieval models could be improved by learning additional high-quality dialogue data.
% However, it is highly labor-intensive to collect high-quality dialogue data in hand-crafted.
% On the other hand, previous studies \cite{adiwardana2020towards, roller2020recipes, brown2020language} demonstrate that well-tuned large-scale generative models show near-human conversation ability.
% % From these observations, we are motivated to use the generation result of these models as a gold response and use as an additional dataset that augments original training dialogue $D$.
% From these observations, we are motivated to augment the dialogue dataset $D$ with responses generated by $\mathcal{G}$ and train retrieval models on the augmented dataset.



%%% Polyencoder까지 있을 때의 Section 2.2

% 5 We first describe our two-staged retrieval-based chatbot pipeline for selecting a response from a pre-defined response set.
% We first describe our retrieval-based conversation pipeline, which consists of the coarse-grained candidate selection stage and fine-grained candidate ranking stage for an efficient manner.
% % The pipeline consists of the coarse-grained candidate selection stage and the fine-grained ranking stage, which is a commonly used architecture for serving Recommender systems \cite{covington2016youtube} or Information Retrieval systems \textcolor{red}{(TODO: Cite)} in an efficient manner.
% Such two-stage pipeline is commonly adopted in recommender \citep{covington2016youtube} and information retrieval [cite] systems where there are a considerable number of possible candidate items (or documents) for the given user (or query).

% \paragraph{Coarse-grained Candidate Selection}{
% % The coarse-grained candidate generation stage produces top-$k$ candidates that could be relevant to the input context.
% The coarse-grained candidate selection stage efficiently searches the top-$k$ response candidates relevant to the given context $c$.
% % We utilized Bi-encoder \cite{humeau2019poly} for encoding the input context and the response candidate.
% We employ Bi-encoder \citep{humeau2019poly} for encoding the given context $c$ and all responses in the pre-defined response repository $R$.
% % As suggested in \citet{humeau2019poly}, we precomputed the embeddings of responses in the pre-defined response set and efficiently searched the candidates using FAISS \cite{johnson2019billion}.
% As suggested in \citet{humeau2019poly}, we first encode responses as embedding vectors based on Bi-encoder and store the embedding vectors at the storage. 
% After that, when a context is given, we also encode the context and efficiently search the top-k response candidates with the fast MIPS library FAISS \cite{johnson2019billion}.
% }

% \paragraph{Fine-grained Candidate Ranking}{
% Poly-encoder \citep{humeau2019poly} captures the richer interaction between the input context and responses through the attention mechanism and therefore has shown better performance than Bi-encoder.
% However, it cannot be used for fast retrieval with fast MIPS libraries due to its complex interaction.
% % We employed Poly-encoder for the ranking of response candidates, which enables richer interactions between the input context and the response compared to the Bi-encoder while retaining a high inference speed.
% % We choose the response with the highest Poly-encoder score among $k$ candidates as the final response.

% Therefore, in the fine-grained candidate ranking stage, we employ Poly-encoder to re-rank the response candidates searched by Bi-encoder.
% Since the size of response candidates $k$ is tiny compared to the total number of responses $n$, Poly-encoder achieves the acceptable inference speed, while it returns the better response among the $k$ response candidates.
% }
% We first describe our efficient retrieval-based conversation pipeline, which consists of the Bi-encoder retrieval model $\mathcal{R}$ and the efficient MIPS library FAISS.
% We employ Bi-encoder \citep{humeau2019poly} for our core retrieval model.
% Bi-encoder encodes the given context $c$ and response $r$ as a fixed-length embedding with Transformer architecture \citep{vaswani2017attention}, and use the dot-product of two embeddings as a score between $c$ and $r$.
% At inference time, we encode all responses in the pre-defined response repository R beforehand to reduce the inference-time latency.
% After that, response with the highest score given context $c$ is selected as a response of the system.

% Since the Bi-encoder uses the dot-product value of two embeddings as the score function, we can utilize efficient maximum inner product search library for speeding up the search process.
% We employ FAISS \citep{johnson2019billion} with Hierarchical Navigable Small World index \citep{malkov2018efficient} because it was empirically found to be fast and accurate.


%%% Model-level G2R PMI 썼을때의 version

% For the model distillation, we employ Mutual Information (MI) \citep{li2015diversity} as a score of the teacher generative model $\mathcal{G}(c, r)$, which is a generalized point-wise mutual information between the given context $c$ and response $r$.
% We choose to use MI score since this score assigns lower score to bland and generic responses and upweight responses that are more informative and more specific to the given context compared to the vanilla log-likelihood score.
% Table \ref{tab:model_level_g2r_example} shows an example that MI score assigns higher values to informative answers and lower values to bland or inappropriate responses.

% We calculate MI score with \textit{MMI-bidi} equation proposed in the original paper, which penalizes the log-likelihood score with the unconditional language model log-likelhood score.
% Since the scale of MI score is affected by the length of responses such as in log-likelihood score \citep{murray2018correcting}, we utilize the length-normalized version of the original score:


% \begin{equation}
%     \mathcal{G}(c, r) = \frac{\log P_{\mathcal{G}}(r|c) - \lambda \log P_{\mathcal{G}}(r)}{|r|}
%     \label{eq:mutual_information}
% \end{equation}
% where $P_\mathcal{G}(r|c)$ is the likelihood of the response $r$ for the input context $c$ of the generative model $\mathcal{G}$, $\lambda$ is a hyperparameter that controls how much to penalize generic responses, and $|r|$ is the number of tokens in $r$.

% However, the language model probability term $P_\mathcal{G}(r)$ in Equation \ref{eq:mutual_information} cannot be obtained since $\mathcal{G}$ is only trained for the situation where the input context $c$ is given. 
% We can obtain this value by either training a separate language model or marginalizing the probabilities over randomly selected contexts.
% Although these options require the training of new language model or require extensive computation, respectively.
% Instead, we employ a simple trick to approximate $P_\mathcal{G}(r)$ by taking the average of the likelihood values of $r$ given dummy input contexts (e.g., \textit{"."}, \textit{"<PAD>"} or \textit{"<UNK>"}).
% This trick enables us to avoid from a burden to train the separate model for calculating a language model probability or calculating an intractable marginal probability.


%% Reference models & Dataset

% \subsection{Reference models \& Dataset}
% We use Blender 9.4B \citep{roller2020recipes} generative model as our large-scale generative model $\mathcal{G}$, and compare the performance of our models against Blender generative models with various network sizes.
% To ensure a fair comparison with these models, we utilize the same datasets that are used to train Blender models, which is the concatenation of Blended Skill Talk \citep{smith2020bst}, ConvAI2 \citep{zhang2018convai2}, Empathetic Dialogues \citep{rashkin2018ed}, and Wizard of Wikipedia \citep{dinan2018wizard}.
% For notational simplicity, we denote the concatenation of these four datasets as BST+.


%%% Model-level G2R ablation
% \subsubsection{Selection of Generator score $G(c, r)$}
% % Generator Score를 PMi 0.5로 하는 것, 1로 하는것, NNLL로 하는 것 끼리 비교
% \input{Tables/Table_Ablation_MD_Loss}
% To analyze the effect of choosing different generator score $G(c, r)$ for model-level G2R, we conduct an ablation study by testing various types of score function by controlling the $\lambda$ value in Equation \ref{eq:model_distillation_loss}.
% Note that using $\lambda=0$ is equivalent to using length-normalized log-likelihood score of the generator model, $\log P_\mathcal{G}(r|c) / |r|$.

% Table \ref{tab:ablation_model_distillation_loss} shows the evaluation result.
% Selecting large $\lambda$ value has an effect of diversifying the selected response, implying that helps to avoid bland and generic responses.
% Using $\lambda=0.5$, the hyperparameter value that we selected, increases the score of human evaluation result compared to vanilla normalized log-likelihood score.
% However, using higher $\lambda$ value rather hurts appropriateness and therefore degrade the performance of the model.




==> Sections/99_Introduction.tex <==
\section{Introduction}\label{sec:1_introduction}
In recent years, with the development of large-scale language models \citep{devlin2019bert,brown2020language}, generative models \citep{sutskever2014sequence,vaswani2017attention,lewis2020bart} have been popular in open-domain conversation \citep{roller2020recipes,zhou2020design,adiwardana2020towards}.
However, existing generative models are too inefficient to be deployed in real-time open-domain conversation systems.
For example, a Blender 9B model \citep{roller2020recipes} requires \textcolor{red}{four GPUs} but could generate only one response per second (1 throughput per second, TPS).
% 작은 모델도 꽤 느리다는 내용 들어갈 수 있을듯

To alleviate this inefficiency, many open-domain conversation systems have employed retrieval models \citep{yoon2018learning,humeau2019poly}, which retrieve responses relevant to the given context  from the pre-defined response repository.
Replacing autoregressive decoding of generative models, retrieval models speed up the response inference time with fast search libraries such as FAISS \citep{johnson2019billion} and FALCON \citep{NIPS2015_2823f479}.
However, retrieval models have a lack of flexibility since they return completely erroneous responses when there are no responses in the pre-defined response repository for the specific context~[cite].

In this paper, to take advantage of each approach, we propose a new learning method of retrieval models by utilizing large-scale generative models from the point of view in knowledge distillation.
Our learning method consists of data- and model-level distillation.
As stated in a previous study~\citep{zhang2020dialoguedistillation}, the performance of retrieval models could be improved by learning additional high-quality dialogue data.
However, collecting high-quality dialogue data is not easy because it usually requires labor-intensive and time-consuming.
Therefore, 
As data-level distillation, 

% Recently, hybrid models \citep{weston2018retrieve,yang2019hybrid,cai2019retrieval} that combine generative models and retrieval models have been proposed to take the advantages of both approaches.
% In hybrid models, based on retrieved responses, generative models produce more informative responses while generating more fluent responses than the retrieved responses.
% Although hybrid models show performance improvement, they suffer from the one-to-many problem [cite] well-known in open-domain conversation where there are many responses for the given context.
% For instance, generative models often ignore retrieved responses when the correspondence between a gold response of the generative models and the retrieved responses is not clear \citep{weston2018retrieve}.



==> Tables/Table_pairwise_human.tex <==
% \begin{table}[h]
% \centering
% \toprule
% \begin{tabular}{@{}cccc@{}}
% \begin{tabular}[c]{@{}l@{}}Model Names\\ \hspace{6pt} (A vs. B)\end{tabular} & A Win & Tie & B Win \\
% \midrule
% Ours vs. Baseline                                               &       &     &       \\
% Ours vs. Blender 90M                                            &       &     &       \\
% Ours vs. Blender 2.7B                                           &       &     &       \\
% Ours vs. Blender 9.4B                                           &       &     &       \\
% Ours vs. Human                                                  &       &     &       \\
% \bottomrule
% \end{tabular}
% \caption{Pairwise human evaluation results.}
% \label{tab:pairwise_human_evaluation}
% \end{table}


\begin{table*}[h]
\centering
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Model names\\ (A vs. B)\end{tabular}} & \multicolumn{3}{c}{Appropriateness} & \multicolumn{3}{c}{Informativeness} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} & A Wins      & Tie      & B Wins     & A Wins      & Tie      & B Wins     \\
\midrule
Ours vs. Blender 90M  & \textbf{34.3\%} & 32.3\% & 33.5\% & 32.9\% & 29.7\% & \textbf{37.4\%} \\
Ours vs. Blender 2.7B & 25.9\% & 33.3\% & \textbf{40.9\%} & 28.4\% & 30.4\% & \textbf{41.3\%} \\
Ours vs. Blender 9.4B & 25.1\% & 36.7\% & \textbf{38.2\%} & 22.0\% & 33.5\% & \textbf{44.5\%} \\
Ours vs. Ours Baseline & \textbf{36.2\%} & 35.4\% & 28.4\% & \textbf{39.4\%} & 31.8\% & 28.8\% \\
Ours vs. Human Response & \textbf{33.3\%} & 36.8\% & 29.9\% & \textbf{35.3\%} & 32.5\% & 32.3\% \\
\bottomrule
\end{tabular}
\caption{Pairwise human evaluation results. [NOTE] Not a valid result.}
\label{tab:pairwise_human_evaluation}
\end{table*}




==> guidelines.tex <==
These instructions are for authors submitting papers to EMNLP 2021 using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} as well as guidelines set forth in the EMNLP 2021 call for papers. This document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{emnlp2021.tex}),
the \LaTeX{} style file used to format it (\texttt{emnlp2021.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{emnlp2021}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{emnlp2021}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
\citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

% Entries for the entire Anthology, followed by custom entries
\bibliography{anthology,custom}
\bibliographystyle{acl_natbib}

\appendix

\section{Example Appendix}
\label{sec:appendix}

This is an appendix.

